Balanced Filtering via Disclosure-Controlled Proxies

We study the problem of collecting a cohort or set that is balanced with respect to sensitive groups when group membership is unavailable or prohibited from use at deployment time. Specifically, our deployment-time collection mechanism does not reveal significantly more about the group membership of any individual sample than can be ascertained from base rates alone. To do this, we study a learner that can use a small set of labeled data to train a proxy function that can later be used for this filtering or selection task. We then associate the range of the proxy function with sampling probabilities; given a new example, we classify it using our proxy function and then select it with probability corresponding to its proxy classification. Importantly, we require that the proxy classification does not reveal significantly more information about the sensitive group membership of any individual example compared to population base rates alone (i.e., the level of disclosure should be controlled) and show that we can find such a proxy in a sample- and oracle-efficient manner. Finally, we experimentally evaluate our algorithm and analyze its generalization properties.

==> non_disclosiveness.tex <==
\subsection{Non-Disclosiveness}

In addition to desiring that the convex hull of our conditional distribution matrix $A$ contains the uniform distribution, we would also like it to be the case that these conditional distributions are not overly disclosiveness. In other words, we do not want to be able to learn \textit{too much} about the sensitive group membership of any individual based on what proxy group they fall into. While there are many ways that we could characterize this diffusion mathematically (entropy, mutual information, etc.), we will ask that for no sensitive group $i$ and proxy $j$ it the case that $P[z=i|g=j] > 1 - \alpha$.
\ed{Update this.}

\begin{definition}[$\alpha$-Disclosive Proxy]
We will say that a proxy $g$ is $\alpha$-disclosive if, for all sensitive groups $i$ and proxy values $j$, $\Pr [z=i|g=k] \leq 1 - \alpha$.
\end{definition}

\begin{mini}|l|
{h\in \Hs}{\sum_i h(x_i) \sum_{k=1}^{K} \1_{z_i = k}\cdot \left(U_k' - U_k\right) }{}{}
\addConstraint{\frac{\sum_i h(x_i) \1_{z_i = k}}{\sum_i h(x_i)}}{\leq 1-\alpha}{\; \forall k}
\addConstraint{\frac{\sum_i (1-h(x_i)) \1_{z_i = k}}{\sum_i (1-h(x_i))}}{\leq 1-\alpha}{\; \forall k}
\addConstraint{f(\gamma) \lVert U - U' \rVert \lVert V - U' \rVert - \langle V_1 - V, U - U' \rangle}{\leq 0}{}
\label{eqn:program}
\end{mini}
